Numerical Discrete-Time Implementation of Continuous-Time Linear-Quadratic Model Predictive Control

This study presents the design, discretization and implementation of the continuous-time linear-quadratic model predictive control (CT-LMPC). The control model of the CT-LMPC is parameterized as transfer functions with time delays, and they are separated into deterministic and stochastic parts for relevant control and filtering algorithms. We formulate time-delay, finite-horizon CT linear-quadratic optimal control problems (LQ-OCPs) for the CT-LMPC. By assuming piece-wise constant inputs and constraints, we present the numerical discretization of the proposed LQ-OCPs and show how to convert the discrete-time (DT) equivalent into a standard quadratic program. The performance of the CT-LMPC is compared with the conventional DT-LMPC algorithm. Our numerical experiments show that, under fixed tunning parameters, the CT-LMPC shows better closed-loop performance as the sampling time increases than the conventional DT-LMPC.

==> tex/NumericalExperiments_JBJO.tex <==
\section{Introduction}
\label{sec:Introduction}
Consdier the optimal control problem (OCP) in Langrange form with piecewise constant inputs
\begin{subequations}
\label{eq:continuousOCP}
\begin{alignat}{5}
    & \min \quad && \phi=\int_{t_0}^{t_0+T} l(t,\tilde z(t)) dt && \\
    & s.t. && x(t_0) = \hat x_0 \\
    & && \dot x(t) = f(t,x(t),u(t)) \, && t \in [t_0, t_0+T] \\
    & && \tilde z(t) = g(t,x(t),u(t)) && t \in [t_0, t_0+T] \\
    & && u(t) = u_k \quad && t \in [t_k, \, t_k+T_s), \, k \in \mathcal{N}
\end{alignat}
\end{subequations}
and the stage cost function
\begin{equation}
l(t,\tilde z(t)) = \frac{1}{2} \norm{ W_c(t) \tilde z(t) }_2^2.
\end{equation}

In Nonlinear Model Predictive Control (NMPC) this problem is solved numerically by solution of
\begin{subequations}
\begin{alignat}{3}
    & \min \quad && \phi= \sum_{k=0}^{N-1} L_k(x_k,u_k) \\
    & s.t. && x_0 = \hat x_0 \\
    & && x_{k+1} = F_k(x_k,u_k) \quad k \in \mathcal{N}
\end{alignat}
\end{subequations}
Sometimes when implicit numerical integrators are used the discrete-time OCP equivalent to \eqref{eq:continuousOCP}
\begin{subequations}
\begin{alignat}{3}
    & \min \quad && \phi= \sum_{k=0}^{N-1} L_k(x_k,x_{k+1},u_k) \\
    & s.t. && x_0 = \hat x_0 \\
    & && R_k(x_k,x_{k+1},u_k) = 0 \quad k \in \mathcal{N}
\end{alignat}
\end{subequations}

Linear-quadratic model predictive control
\begin{subequations}
\begin{alignat}{3}
    & \min \quad && \phi=\int_{t_0}^{t_0+T} l(t,\tilde z(t)) dt \\
    & s.t. && x(t_0) = \hat x_0 \\
    & && \dot x(t) = A_c x(t) + B_c u(t) + b(t), \, t \in [t_0, t_0+T] \\
    &&& \tilde z(t) = C_c x(t) + D_c u(t) + c(t) \\
    & && u(t) = u_k \quad t \in [t_k, \, t_k+T_s), \, k \in \mathcal{N}
\end{alignat}
\end{subequations}


\begin{subequations}
\begin{alignat}{3}
    & \min \quad && \phi= \sum_{k=0}^{N-1} L_k(x_k,u_k) \\
    & s.t. && x_0 = \hat x_0 \\
    & && x_{k+1} = A x_k + B u_k + b_k  \quad k \in \mathcal{N}
\end{alignat}
\end{subequations}

\begin{equation}
L_k(x_k,u_k) = \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' \begin{bmatrix} Q_{xx} & Q_{xu} \\ Q_{ux} & Q_{uu} \end{bmatrix} \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \begin{bmatrix} q_{x,k} \\ q_{u,k} \end{bmatrix}'\begin{bmatrix} x_k \\ u_k \end{bmatrix} + \gamma_k 
\end{equation}


\begin{equation}
Z(s) = G(s) U(s)
\end{equation}

